Convergence of Two-Layer Regression with Nonlinear Units

Large language models (LLMs), such as ChatGPT and GPT4, have shown outstanding performance in many human life task. Attention computation plays an important role in training LLMs. Softmax unit and ReLU unit are the key structure in attention computation. Inspired by them, we put forward a softmax ReLU regression problem. Generally speaking, our goal is to find an optimal solution to the regression problem involving the ReLU unit. In this work, we calculate a close form representation for the Hessian of the loss function. Under certain assumptions, we prove the Lipschitz continuous and the PSDness of the Hessian. Then, we introduce an greedy algorithm based on approximate Newton method, which converges in the sense of the distance to optimal solution. Last, We relax the Lipschitz condition and prove the convergence in the sense of loss value.

==> related_work_addition.tex <==
\subsection{Additional related-work}
We introduce some additional related-work on LLMs in this section.

\paragraph{Upon practical LLMs} Recently, we have witnessed an explosive amount research on practical LLMs. Researchers have been focused on evaluating the capability of chat-GPT \cite{qzz+23,gzx+23,zll+23,bcl+23} and GPT-4 \cite{o23, bce+23}. multi-task processing, capability in different areas (ex. coding, mathematics, philosophy, and etc.), limitation - hallucinogen problems, sentence tugging
\cite{tli+23} 
